Soft-Phonon-Driven Effective Inversion-Symmetry Crossover in Quantum Paraelectrics

Symmetry lays the foundation of condensed matter physics and its experimental manifestation provides fundamental insight into the collective behaviors of quantum materials. Optical second-harmonic generation (SHG) is widely regarded as a fingerprint of inversion-symmetry breaking, yet whether and how collective lattice dynamics govern the nonlinear optical manifestation of local inversion-symmetry breaking remains unknown. Here, combining optical SHG, diffuse X-ray scattering, and microscopic theory, we reveal a phonon-regulated mechanism governing the temperature-dependent manifestation of local inversion-symmetry breaking in quantum paraelectric material KTaO3. We demonstrate that an oxygen-defect-mediated nonlinear optical channel is strongly coupled to the host soft polar mode, whose thermal fluctuations scramble the associated electronic phase coherence and thereby suppress the nonlinear manifestation of local inversion-symmetry breaking at elevated temperatures. Consequently, the nonlinear response exhibits a temperature-driven crossover from a regime in which local inversion-symmetry breaking is optically manifest to one that appears effectively centrosymmetric, without any accompanying structural change. Our findings revise the conventional picture of the temperature-dependent manifestation of inversion-symmetry breaking in quantum paraelectrics and establish a framework for understanding and engineering defect-mediated nonlinear optical responses in materials hosting low-energy polar excitations.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeaux' );
sub makeaux {
    my ($base, $ext) = @_;
    system("pdflatex -synctex=1 -interaction=nonstopmode \"$base\"");
}

